AmbigDocs: Reasoning across Documents on Different Entities under the Same Name

Different entities with the same name can be difficult to distinguish. Handling confusing entity mentions is a crucial skill for language models (LMs). For example, given the question "Where was Michael Jordan educated?" and a set of documents discussing different people named Michael Jordan, can LMs distinguish entity mentions to generate a cohesive answer to the question? To test this ability, we introduce a new benchmark, AmbigDocs. By leveraging Wikipedia's disambiguation pages, we identify a set of documents, belonging to different entities who share an ambiguous name. From these documents, we generate questions containing an ambiguous name and their corresponding sets of answers. Our analysis reveals that current state-of-the-art models often yield ambiguous answers or incorrectly merge information belonging to different entities. We establish an ontology categorizing four types of incomplete answers and automatic evaluation metrics to identify such categories. We lay the foundation for future work on reasoning across multiple documents with ambiguous entities.

==> extra.tex <==
\section{Summary}

% Thanks to RAG, we can simply concatenate retrieved documents and let LLM do multi-document reasoning with a single prompt. This allows tasks that span multiple documents like multi-answer / multi-hop QA and summarization to perform well without finetuning or additional modules for measuring interactions. However, a challenge arises when the query contains an ambiguous entity, conveying additional burden of distinguishing retrieved documents of different entities to the LM.

% We showcase this issue actually happens in QA task. It does get better with complex task-specific prompting, but model should do this without. Our method does this without elaborate prompting.

% Among tasks involving multi-documents, we focus on ambiguous QA, which requires recognizing potential disambiguations and finding all appropriate answers, necessitating deep understanding of the documents. Particularly, we explore one subset of ambiguous questions, \texttt{Entity References}, defined as follow: ``There is a noun phrase in the question which may be resolved in multiple ways". While the answers from other types \footnote{\texttt{Conditional} (63\%): question needs to be specified with additional conditions, \texttt{Underspecified Type} (16\%): missing the type of desired answer, \texttt{Time Dependent} (13\%): answer depends on time at which question was asked} are mainly from a single event or non-ambiguous pages, only 23\% of the questions are about entity ambiguity, which requires additional burden mentioned above.

% We start with principle ``Wikipedia ambiguous entity can be interpreted as each entity in its disambiguation page" and ``the noun phrase (ambiguous entity) can be substituted by Wikipedia disambiguation to serve as a dismabiguated question”. Since there are around 200,000 ambiguous entities, we create a large-scale synthetic dataset covering rare entities to encourage further research.
% Moreover, we start with some confusing passages to generate questions, not from (NQ) questions then visiting potential passages, hence we annotate the gold passage for each disambiguated answer (AmbigQA provides only underestimation, and ASQA provides only 45\%). Lastly, we classify the disambiguation types as (1) AE is inside DEs (e.g. Oregon, Illinois, Oregon, Kentucky), (2) AE is not inside DEs (e.g. Chungmugong Yi Sun-sin class destroyer, Chungmuro), (3) AE is inside only one DE (Don Carlos (basketball), Charles III of Spain) or (Chokha, Chukha District). Also, by the types -- it seems human names / locations are easier.

(Unsure) We examine how current models react to our dataset and provide a simple method for better performance...

However, a recent work \cite{Chiang2024MergingFC} has shown that open-source LMs suffer from distinguishing passages of ambiguous names for biography generation. In this paper, we delve into making the LM robust at such passage confusions, with a focus on ambiguous QA task.

We simulate this setting by starting with two passages where the titles (entities) are disambiguated from an ambiguous entity AE. We generate a question about the AE, which to be interpreted differently by each passage. In addition, we generate a short answer for each passage and a comprehensive long answer to ensure the question is ambiguous and filter out the failures.

\begin{table}[t]
\begin{center}
\begin{tabular}{p{5cm} p{8cm}}
\toprule
\multicolumn{2}{l}{\bf Example}\\
\midrule
\multicolumn{2}{l}{Q: What does ``\textcolor{red}{Write-only memory}" refer to?} \\
DE1: Write-only memory (engineering) & Ans: A memory location or register that can be written to but not read \\
DE2: Write-only memory (joke) & Ans: A joke or a euphemism for a failed memory device \\ \midrule
% \multicolumn{2}{l}{Q: What was the profession of \textcolor{red}{William Hurst}?} \\
% DE1: William John Hurst & Ans: Member of Parliament in New Zealand and Mayor of Auckland \\
% DE2: William Hurst (civil engineer) & Ans: Civil engineer \\
% DE3: Bill Hurst & Ans: Former Major League Baseball player \\
% DE4: William C. Hurst & Ans: Extension Specialist and Professor of Food Science and Technology \\ \midrule
% \multicolumn{2}{l}{Q: Where is \textcolor{red}{Yeshiva University High School} located?} \\
% DE1: Marsha Stern Talmudical Academy & Ans: Washington Heights neighborhood in the New York City borough of Manhattan \\
% DE2: Yeshiva University High School for Girls & Ans: Holliswood, in the New York City borough of Queens \\ \midrule
\multicolumn{2}{l}{Q: What is the population of  \textcolor{red}{Fitzpaine} according to the 2011 census?} \\
DE1: Okeford Fitzpaine & Ans: 913 \\
DE2: Wootton Fitzpaine & Ans: 345 \\
DE3: Cheriton Fitzpaine & Ans: 556 \\ \midrule
% \multicolumn{2}{l}{Q: What is the seating capacity of \textcolor{red}{Starduster}?} \\
% DE1: Stolp Starduster & Ans: single seat \\
% DE2: Stolp Starduster Too & Ans: two-seat \\ \midrule
\multicolumn{2}{l}{Q: Who primarily uses ``\textcolor{red}{The Joe}" as their playing field?} \\
DE1: Joseph L. Bruno Stadium & Ans: Tri-City ValleyCats minor league baseball team \\
DE2: Sewell-Thomas Stadium & Ans: University of Alabama Crimson Tide college baseball team \\
DE3: Joe Louis Arena & Ans: Detroit Red Wings of the National Hockey League \\ \midrule
% \multicolumn{2}{l}{Q: Who founded the \textcolor{red}{Boston Store}?} \\
% DE1: J. L. Brandeis and Sons & Ans: Jonas L. Brandeis \\
% DE2: J. W. Robinson's & Ans: Joseph Winchester Robinson \\
% DE3: Edgar Department Stores & Ans: James Edgar \\
% DE4: Sibley's & Ans: Rufus Sibley, Alexander Lindsay, and John Curr \\
\bottomrule
\end{tabular}
\end{center}
\caption{Examples from our dataset. Ambiguous entity is coloured in red inside the question. Below the question, disambiguated entities are paired with their answers to the question.\ec{we need to show that we have *passages* as that's the main difference from prior work}}
\label{tab:data_example}
\end{table}

\begin{table}[t]
\begin{center}
\begin{tabular}{p{2cm}p{11cm}}
\toprule
\multicolumn{2}{l}{Q: Where is footballer \textcolor{red}{Walter Andrade} from?} \\ \midrule
Llama2 & Walter Andrade is from \textcolor{blue}{Peru} and \textcolor{purple}{Argentina}. \\ \midrule
GPT-3.5 & Footballer Walter Andrade is from \textcolor{purple}{Argentina}. \\ \midrule
GPT-4 & There are two footballers named Walter Andrade. \textcolor{blue}{Walter William Andrade Zevallos, born in 1982, is from Peru}. \textcolor{purple}{Walter Saúl Andrade, born in 1984, is from Argentina}. \\
\bottomrule
\end{tabular}
\end{center}
\caption{Examples of generated answers, varying on different LMs. Answer for $DE_1$ and $DE_2$ is coloured in blue and purple, respectively. \ys{Will change the example}}
\label{tab:error_types}
\end{table}

\begin{table}[t]
\begin{center}
\begin{tabular}{l}
\toprule
Q: What is the population of \textcolor{red}{Fitzpaine} according to the 2011 census? \\ \midrule
DE1: Okeford Fitzpaine \\
Passage (3919760): Okeford Fitzpaine is a ... In the 2011 census ... a population of 913 ... \\
Answer 1: 913 \\ \midrule
DE2: Wootton Fitzpaine \\
Passage (3929977): Wotton Fitzpaine is a ... In the 2011 census ... a population of 345 ... \\
Answer 2: 345 \\ \midrule
DE3: Cheriton Fitzpaine \\
Passage (6913024): Cheriton Fitzpaine is a ... The poplutaion ... 2011 census was 556 ... \\
Answer 3: 556 \\ 
\bottomrule
\end{tabular}
\end{center}
\caption{Example of our dataset. The ambiguous entity is coloured in red inside the question. Below the question is a list containing answers of multiple disambiguations of the shared entity. Each answer is paired with a gold passage where it was found.
\ec{we need to show that we have *passages* as that's the main difference from prior work}}
\label{tab:data_example}
\end{table}

We leverage variants of EAR metric to quantify \textit{Partial}, \textit{Nonfactual}, and \textit{Complete} behaviours of LLMs. The scores are each averaged amongst the test split. \(max_k/min_k\) indicates the $kth$ largest/smallest element.
\begin{itemize}
    \item \textbf{Complete}\((Q_{AE})=min_1 \{{R(DE^{uniq}_i)R(Ans_i)\}}\). If the model got all answers correct, the minimum of the scores will also be high. \(Complete(Q_{AE})\) reduces the effect of partial credits and measure how much complete answer the model has generated. 
    \item \textbf{Partial}\((Q_{AE})=max_1 \{{R(DE^{uniq}_i)R(Ans_i)\}} - min_1 \{{R(DE^{uniq}_i)(Ans_i)\}}\). We observe the difference between the maximum and minimum score for each answer. \(Partial(Q_{AE})\) being high indicates the model has found some of the answers.
    \item \textbf{Ambiguous}\((Q_{AE})=max_1 \{(1-R(DE^{uniq}_i))R(Ans_i)\}-max_2 \{(1-R(DE^{uniq}_i))R(Ans_i)\}\). Existence of answers without entity indications are problematic. In other words, if $R(DE^{uniq}_i)$ is low and $Rec(Ans_i)$ is high, the product will capture such behaviour. There should be only one answer, so we observe the difference between the largest and second largest score.
    \item \textbf{Merged}\((Q_{AE})=max_2 \{(1-R(DE^{uniq}_i))R(Ans_i)\}\). We observe the same product as \textit{Ambiguous} case. However, there should be more than two answers, so we observe the second largest score. 
\end{itemize}

\subsection{Manual Inspection Results}

\begin{figure}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{Template-2024/assets/manual.png}
\end{center}
\caption{Results of manually inspecting 100 questions under \textbf{All Gold} experiment.}
\label{fig:manual}
\end{figure}

We manually assess 100 questions under \textsc{All Gold} setting. The results are presented in Figure \ref{fig:manual}. We observe the rankings among the models are preserved within \textit{Nonfactual} and \textit{Complete} metrics. For \textit{Partial} metric, the trend is still preserved. Yet, while the manual count being binary, the actual magnitude of the metric depends on the maximum score of the answer set. We find that better LMs (Mistral, GPT-4) exhibit higher maximum score compared to Llama2-13b and GPT-3.5, resulting a higher \textit{Partial} score as opposed to naive counting.

A standard metric for evaluating the generated answer $Ans_{AE}$ for $Q_{AE}$ is to average the token-level recall scores of each gold answer $Ans_i$, i.e. \(Ans(Q_{AE}) = \frac{1}{n}\sum{R(Ans_i)}\), where \(R(Ans_i)\) stands for recall of $Ans_i$ to $Ans_{AE}$. However, according to this metric, the model is not required to distinguish distinct entities. To mitigate this, we introduce a weighing factor $f(i)$ to be multiplied to the score of each answer, which reduces the effect of $Ans_i$ if $DE_i$ is not present. Precisely, we define $DE^{uniq}_i$ as the \textit{unique identifier} of $DE_i$ by removing all token-level overlaps with $AE$. Considering $f(i) = R(DE^{uniq}_i)$, the score for each answer will remain high only if successfully paired with its entity.\footnote{There may be an answer like `$DE_i$ is $Ans_j$ and $DE_j$ is $Ans_i$', which exploits the metric design. Nevertheless, we have never seen such case when manually inspecting 100 outputs for each experiment. Generally speaking, our metric assumes that LM does not cross the answers.} Then, EAR score for $Q_{AE}$ is calculated as follows, \(EAR(Q_{AE}) = \frac{1}{n}\sum{R(DE^{uniq}_i)R(Ans_i)}\), and the scores are averaged amongst the test questions to obtain the final EAR score of test split.

% We should expect the model to not only find all possible answers in the retrieved context, but also distinguish different entities as a \textbf{Complete} answer. However, the model may fail to discover the full answer list, resulting a \textbf{Partial} answer. In addition, the model recognize only one entity among the passages, resulting \textbf{Partial} answer. Moreover, the model may fail to distinguish two entities and mix up the answers, leading to {\bf Nonfactual} generation. Lastly, the model sometimes refuses to answer, which is a \textbf{Failure} case.

\subsubsection{Quantifier Metrics}
EAR score decomposes correctness of the generated answer of an LM into two components, $R(DE^{uniq}_i)$ and $R(Ans_i)$. We leverage this breakdown to quantify five behaviours observed in Section \ref{sec:manual}. The follow process decides which class $Ans_{AE}$ should belong at.

We first determine \textit{Ambiguous} and \textit{Merged} behaviours. Both cases deal with the existence of an answer without entity indication. To capture such behaviour, we count the number of gold answers where $R(Ans_i) > 0.2$\footnote{We set a nonzero threshold to ignore not meaningful tokens such as stopwords.} and $R(DE^{uniq}_i)=0$. If the count equals to one, $Ans_{AE}$ is classified as \textit{Ambiguous}, otherwise, $Ans_{AE}$ is classified as \textit{Merged}.

Next, we count the number of gold answers where $R(Ans_i) > 0.2$ and $R(DE^{uniq}_i)>0$. If the count equals the number of gold answer set, the model has generated \textit{Complete} answer. If the count is greater or equal than one, the model has generated \textit{Partial} answer. Otherwise, we label as \textit{Failure}, which means $R(Ans_i) <= 0.2$ for all answers.

\begin{itemize}
    \item \textbf{Complete}: The model found all answers correctly and distinguished the entity for each answer, i.e. all $Ans_i$ is paired with $DE_i$.
    \item \textbf{Partial}: The model found partial answers correctly and distinguished distinct entities, i.e. some answer $Ans_i$ is paired with $DE_i$.
    \item \textbf{Ambiguous}: The model found one answer but did not provide the specific entity, i.e. the answer is paired with ambiguous entity $AE$ or no entity.
    \item \textbf{Failure}: The model did not find any correct answers.
    \item \textbf{Merged}: The model found multiple answers but merged all entities, i.e. all answers are paired with ambiguous entity $AE$.
\end{itemize}

\begin{table}[t]
\begin{center}
\begin{tabular}{l|c|c|c|c|c}
\toprule
 & Llama2-7b & Mistral-7b & Llama2-13b & GPT-3.5 & GPT-4 \\ \midrule
\multicolumn{6}{c}{\textit{Entity-Answer Recall}} \\ \midrule
\textsc{All Gold} & 0.384 & \underline{0.481}& 0.253 & 0.241 & \textbf{0.484} \\
\textsc{Gold+Retrieved} & 0.372 & \textbf{0.410} & 0.230 & 0.207 & \underline{0.374} \\
\textsc{All Retrieved} & 0.216 & \textbf{0.267} & 0.150 & 0.158 & \underline{0.234} \\
\midrule
\multicolumn{6}{c}{\textit{Disambig-F1}} \\ \midrule
\textsc{All Gold} & 0.215 & \underline{0.242} & 0.176 & 0.176 & \textbf{0.287} \\
\textsc{Gold+Retrieved} & 0.186 & \underline{0.195} & 0.144 & 0.150 & \textbf{0.218} \\
\textsc{All Retrieved} & 0.115 & \underline{0.134} & 0.106 & 0.120 & \textbf{0.146} \\
\midrule
\multicolumn{6}{c}{\textit{Answer Recall}} \\ \midrule
\textsc{All Gold} & 0.559 & \underline{0.592} & 0.466 & 0.421 & \textbf{0.654} \\
\textsc{Gold+Retrieved} & \underline{0.528} & 0.523 & 0.415 & 0.371 & \textbf{0.542} \\
\textsc{All Retrieved} & 0.385 & \underline{0.404} & 0.322 & 0.318 & \textbf{0.406} \\
\midrule
\multicolumn{6}{c}{\textit{Unique Entity Recall}} \\ \midrule
\textsc{All Gold} & 0.534 & \textbf{0.650} & 0.382 & 0.362 & \underline{0.602} \\
\textsc{Gold+Retrieved} & \underline{0.529} & \textbf{0.579} & 0.363 & 0.332 & 0.493 \\
\textsc{All Retrieved} & 0.365 & \textbf{0.430} & 0.275 & 0.278 & \underline{0.372} \\
\midrule
\multicolumn{6}{c}{\textit{Answer Length}} \\ \midrule
\textsc{All Gold} & 985.5 & 1007.4 & 594.0 & 327.4 & 728.8 \\
\textsc{Gold+Retrieved} & 1231.7 & 1098.5 & 655.9 & 337.9 & 750.6 \\
\textsc{All Retrieved} & 1157.7 & 1083.9 & 608.5 & 334.1 & 703.4 \\
\bottomrule
\end{tabular}
\end{center}
\caption{Experimental results.}
\label{tab:results_allgold}
\end{table}

\begin{itemize}[leftmargin=*]
    \item \textbf{Complete} (+2): The model correctly identifies all answers and distinguishes the entity for each answer, i.e. $c_p=n$.
    % In other words, for all $i$, $ R(Ans_i)\geq \tau_A$ and $R(DE^{uniq}_i)\geq \tau_E$. 
    % (All $Ans_i$ are paired with $DE_i$)
    \item \textbf{Partial} (+1): The model correctly identifies partial answers and distinguishes those entities, i.e. $1\leq c_p<n$.
    % That is, for some $i$, $ R(Ans_i)\geq \tau_A$ and $R(DE^{uniq}_i)\geq \tau_E$. 
    % (Some $Ans_i$ are paired with $DE_i$)
    \item \textbf{Failure} (+0): The model fails to identify any correct answers, i.e. $c_p=c_{np}=0$.
    % That is, for all $i$, $R(Ans_i)< \tau_A$.
    \item \textbf{Ambiguous} (-1): The model identifies exactly one answer but provides an ambiguous entity or no entity, i.e. $c_p=0$ and $c_{np}=1$.
    % That is, for only one $i$, $ R(Ans_i)\geq \tau_A$, and for such $i$, $R(DE^{uniq}_i)< \tau_E$. 
    % (The answer is paired with $AE$ or no entity)
    \item \textbf{Merged} (-2): The model identifies multiple answers but merges the entities, i.e. $2\leq c_{np} \leq n$.
    % In other words, for more than one $i$, $ R(Ans_i)\geq \tau_A$ and $R(DE^{uniq}_i)< \tau_E$. 
    % (Multiple answers are paired with $AE$)
\end{itemize}

\begin{table}[t]
\begin{center}
\begin{tabular}{l|c|c|c|c|c}
\toprule
& Answer Recall & Entity Recall & Entity-Answer Recall & Disambig-F1 \\ \midrule
Llama2-7b & 0.453 \textcolor{red}{(-.079)} & 0.427 \textcolor{red}{(-.077)}& 0.284 \textcolor{red}{(-.077)}& 0.201 \textcolor{red}{(-.006)} \\
Mistral-7b & 0.593 \textcolor{blue}{(+.035)} & 0.713 \textcolor{blue}{(+.083)} & 0.499 \textcolor{blue}{(+.039)} & 0.283 \textcolor{blue}{(+.048)} \\
Llama2-13b & 0.464 \textcolor{blue}{(+.026)} & 0.422 \textcolor{blue}{(+.076)} & 0.280 \textcolor{blue}{(+.047)} & 0.205 \textcolor{blue}{(+.036)}  \\
GPT-3.5 & 0.407 \textcolor{blue}{(+.015)} & 0.379 \textcolor{blue}{(+.049)} & 0.267 \textcolor{blue}{(+.040)} & 0.192 \textcolor{blue}{(+.022)} \\
GPT-4 & 0.723 \textcolor{blue}{(+.095)} & 0.787 \textcolor{blue}{(+.205)} & 0.640 \textcolor{blue}{(+.175)} & 0.363 \textcolor{blue}{(+.090)} \\
\bottomrule
\end{tabular}
\end{center}
\caption{Few-shot results. We provide the difference from zero-shot result in the paranthesis. }
\label{tab:few}
\end{table}

% We consider the answer has been correctly identified if we find a token of $a^*_i$ in $y$, excluding the tokens commonly appearing the entire answer set.\footnote{If $a^*_i$ is '2017 horror film' and token 'film' appears in all other answers, we consider it as correct only if '2017' or 'horror' is present in $y$. Precisely, for $a^*_i=(w_{i_1}, \dots, w_{i_t})$ and the set of common tokens $S=\cap_j \{w_{j_k}\}$, $\tau_{a_i}=\max(|S|/t, 0.15)$ (We prevent threshold from being too low).} 

\begin{table}[t]
\begin{center}
\begin{tabular}{p{38em}}
\toprule \toprule
$q_{sn}$: When was \textbf{Nengren Temple} first established? \\ \midrule
$DE^*_1$: Nengren Temple (Guangzhou) \\
$d^*_1$: Nengren Temple (Guangzhou) Nengren Temple () is a Buddhist temple located ... was first established by Yinjian () in \textbf{1824}, during the reign of Daoguang Emperor (1821-1850) of the Qing dynasty (1644-1911). ... \\ 
$a^*_1$: 1824 \\ \midrule
$DE^*_2$: Nengren Temple (Jiujiang) \\
$d^*_2$: Nengren Temple (Jiujiang) Nengren Temple () is a Buddhist temple located ... was first built in the \textbf{Northern and Southern dynasties (420-589)}, and went through many changes and repairs through the following dynasties. ... \\
$a^*_2$: Northern and Southern dynasties (420-589) \\ \midrule \midrule
$q_{sn}$: What is the primary function of the \textbf{Pollicis brevis muscle}? \\ \midrule
$DE^*_1$: Abductor pollicis brevis muscle \\
$d^*_1$: Abductor pollicis brevis muscle ... is a muscle in the hand that functions as an \textbf{abductor of the thumb}. ... \\
$a^*_1$: An abductor of the thumb \\ \midrule
$DE^*_2$: Flexor pollicis brevis muscle \\
$d^*_2$: Flexor pollicis brevis muscle ... is a muscle in the hand that \textbf{flexes the thumb}. ... \\ 
$a^*_2$: Flexes the thumb \\ \midrule 
$DE^*_3$: Extensor pollicis brevis muscle \\
$d^*_3$: first phalanx of the thumb. ... the extensor pollicis brevis both \textbf{extends and abducts the thumb at the carpometacarpal and metacarpophalangeal joints}. ... \\
$a^*_3$: Extends and abducts the thumb at the carpometacarpal and metacarpophalangeal joints \\ \midrule \midrule
$q_{sn}$: Who are the parents of \textbf{Prince Joachim}? \\ \midrule
$DE^*_1$: Prince Joachim of Belgium, Archduke of Austria-Este \\
$d^*_1$ Prince Joachim of Belgium, Archduke of Austria-Este ... is the younger son and third child of \textbf{Lorenz, Archduke of Austria-Este and Princess Astrid of Belgium}. ... \\ 
$a^*_1$: Lorenz, Archduke of Austria-Este and Princess Astrid of Belgium \\ \midrule
$DE^*_2$: Prince Joachim of Denmark\\
$d^*_2$: Prince Joachim of Denmark ... is the younger son of \textbf{Queen Margrethe II and the late Prince Henrik}. ... \\
$a^*_2$: Queen Margrethe II and the late Prince Henrik \\ \midrule
$DE^*_3$: Prince Joachim Albert of Prussia\\
$d^*_3$: Prince Joachim Albert of Prussia ... was the second eldest son of \textbf{Prince Albert of Prussia and his wife Princess Marie of Saxe-Altenburg}. ... \\ 
$a^*_3$: Prince Albert of Prussia and Princess Marie of Saxe-Altenburg \\ \midrule
$DE^*_4$: Prince Joachim of Prussia \\
$d^*_4$: Prince Joachim of Prussia ... was the youngest son of \textbf{Wilhelm II, German Emperor, by his first wife, Augusta Victoria of Schleswig-Holstein}. ... \\ 
$a^*_4$: Wilhelm II, German Emperor and Augusta Victoria of Schleswig-Holstein \\
\bottomrule \bottomrule
\end{tabular}
\end{center}
\caption{Three examples from our dataset. We present the question first, where the bold text in the question indicates the surface name $sn$. Below the question, we present the pairs of $\{DE^*_i, d^*_i, a^*_i\}$. Bold text in each document indicates the evidence for its corresponding answer.}
\label{tab:examples}
\end{table}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

